Classification robustness to common optical aberrations

Computer vision using deep neural networks (DNNs) has brought about seminal changes in people's lives. Applications range from automotive, face recognition in the security industry, to industrial process monitoring. In some cases, DNNs infer even in safety-critical situations. Therefore, for practical applications, DNNs have to behave in a robust way to disturbances such as noise, pixelation, or blur. Blur directly impacts the performance of DNNs, which are often approximated as a disk-shaped kernel to model defocus. However, optics suggests that there are different kernel shapes depending on wavelength and location caused by optical aberrations. In practice, as the optical quality of a lens decreases, such aberrations increase. This paper proposes OpticsBench, a benchmark for investigating robustness to realistic, practically relevant optical blur effects. Each corruption represents an optical aberration (coma, astigmatism, spherical, trefoil) derived from Zernike Polynomials. Experiments on ImageNet show that for a variety of different pre-trained DNNs, the performance varies strongly compared to disk-shaped kernels, indicating the necessity of considering realistic image degradations. In addition, we show on ImageNet-100 with OpticsAugment that robustness can be increased by using optical kernels as data augmentation. Compared to a conventionally trained ResNeXt50, training with OpticsAugment achieves an average performance gain of 21.7% points on OpticsBench and 6.8% points on 2D common corruptions.

==> supp_additional.tex <==
%%%%%%%%%%%%%%%%%%%%% deprecated %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\iffalse
\clearpage

\begin{figure}[h]
    \centering
\includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_refvar_alexnet_drefvar_val.pdf}
    \caption{Corruption error metric as from Hendrycks et al. All severities and DNNs. Color groups represent the different corruptions.}
    \label{fig:my_label}
\end{figure}


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_mode_defocus_blurrefvar_val.pdf}
    \caption{Relative accuracy of defocus blur to clean data. Inset values: Maximum and standard deviation. $100\%$ means equal values.}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_mode_trefoilrefvar_val.pdf}
    \caption{Relative accuracy of trefoil to clean data.}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptionsrefvar_val.pdf}
    \caption{Relative accuracy of all corruptions to clean data.}
    \label{fig:my_label}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptionsrefvar_defocus_blur.pdf}
    \caption{Relative accuracy of all corruptions compared to defocus blur (without clean data).}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_mode_defocus_blurrefvar_alexnet.pdf}
    \caption{Defocus blur (Hendrycks et al.) vs. severity normed to AlexNet acc.}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_mode_astigmatismrefvar_alexnet.pdf}
    \caption{Astigmatism vs. severity normed to AlexNet acc.}
    \label{fig:my_label}
\end{figure}

\begin{figure}
    \centering \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_mode_comarefvar_alexnet.pdf}
    \caption{Coma vs. severity normed to AlexNet acc.}
    \label{fig:my_label}
\end{figure}

\clearpage
%
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_mode_defocus_sphericalrefvar_defocus_blur.pdf}
    \caption{Relative accuracy of spherical and defocus to Hendrycks et al. defocus blur.}
    \label{fig:my_label}
\end{figure}
%
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_mode_astigmatismrefvar_defocus_blur.pdf}
    \caption{Relative accuracy of astigmatism to defocus blur.}
    \label{fig:my_label}
\end{figure}
%
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_mode_comarefvar_defocus_blur.pdf}
    \caption{Relative accuracy for coma and defocus blur.}
    \label{fig:my_label}
\end{figure}
%
%%%%%%%%%%%% kernel report (experimental)
%
\begin{figure}[h]
    \centering
    \includegraphics[page=10,width=\linewidth]{figures/matching/report_sheets_final_cooke_rgb.pdf}
    \caption{Geometric defocus blur from Hendrycks et al. vs. PSF defocus blur and chromatic aberration.}
    \label{fig:my_label}
\end{figure}
%
\begin{figure}[h]
    \centering
    \includegraphics[page=19,width=\linewidth]{figures/matching/report_sheets_final_cooke_rgb.pdf}
    \caption{Geometric defocus blur from Hendrycks et al. vs. astigmatic lens model.}
    \label{fig:my_label}
\end{figure}
%
\begin{figure}[h]
    \centering
    \includegraphics[page=25,width=\linewidth]{figures/matching/report_sheets_final_cooke_rgb.pdf}
    \caption{Geometric defocus blur from Hendrycks et al. vs. coma aberration, severity 5.}
    \label{fig:my_label}
\end{figure}
%
\
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_mode_trefoilrefvar_defocus_blur.pdf}
    \caption{Relative accuracy for trefoil and defocus blur.}
    \label{fig:my_label}
\end{figure}


\newpage

\begin{figure}[h]
    \centering
    \includegraphics[page=39,width=\linewidth]{figures/matching/report_sheets_final_cooke_rgb.pdf}
    \caption{Geometric defocus blur from Hendrycks et al. vs. trefoil aberration.}
    \label{fig:my_label}
\end{figure}



\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rg/report_acc_over_severitysplit_corruptions_refvar_sub_defocus_blur.pdf}
    \caption{Difference in accuracy compared to defocus blur. Color groups represent the different corruptions.}
    \label{fig:my_label}
\end{figure}
\fi



\iffalse
\begin{figure}
    \centering    
    \includegraphics[width=\linewidth]{figures/imagenet100/eval_rgb/report_rank_baseline_trefoil_severity5.pdf}
    \caption{Ranking comparison of baseline (here: astigmatism) and coma for severity 5. The DNNs with pre-computed augmentation on ImageNet-100 achieve better results than the ones without any augmentation during training.}
    \label{fig:my_label}
\end{figure}
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%% (intended for) %%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%% supplementary %%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%  submission due 15th of march %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% https://iccv2023.thecvf.com/submission.guidelines-361600-2-20-16.php 
\iffalse
\newpage
\section{ImageNet100 and ImageNet100-C}
\label{app:imagenet100_and_c}
\begin{figure}[h]
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_highlight_resnet101_sgd_clean_resnet101_sgd_opticsaugment.pdf}
    \caption{ResNet101 clean (red) vs. OpticsAugment (blue).}
    \label{fig:common2d_modes_opticsaugment_resnet101}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_highlight_efficientnet_b0_sgd_clean_efficientnet_b0_sgd_opticsaugment.pdf}
    \caption{EfficientNet clean (red) vs. OpticsAugment (blue).}
    \label{fig:common2d_modes_opticsaugment_efficientnet}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_highlight_mobilenet_v3_large__clean_mobilenet_v3_large__opticsaugment.pdf}
    \caption{MobileNet\_v3 clean (red) vs. OpticsAugment (blue).}
    \label{fig:common2d_modes_opticsaugment_mobilenet}
\end{subfigure}\begin{subfigure}{\linewidth}
    \centering
    \includegraphics[trim=2cm 8.3cm 0.5cm 0cm,clip,width=0.9\linewidth]{figures/imagenet100-c/eval_rgb/labels_only_severity_split.pdf}
    \caption{Selected 2D common corruptions.}
\end{subfigure}
    \caption{Evaluation of 2D common corruptions for the DNNs trained on ImageNet-100 with and without OpticsAugment. }
    \label{fig:common2d_modes_appendix}
\end{figure}


%%%%%%%%%%%%%%%%% ResNet101 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_clean_resnet101.pdf}
    \caption{Highlighted: ResNet101 clean (no augmentation)}
    \label{fig:common2d_modes_clean}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_opticsaugment_resnet101.pdf}
    \caption{Highlighted: ResNet101 clean + OpticsAugment}
    \label{fig:common2d_modes_opticsaugment}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[trim=2cm 8.3cm 0.5cm 0cm,clip,width=0.9\linewidth]{figures/imagenet100-c/eval_rgb/labels_only_severity_split.pdf}
    \caption{2D common corruptions evaluated in Fig.~\ref{fig:common2d_modes_clean} and Fig.~\ref{fig:common2d_modes_opticsaugment}.}
\end{subfigure}
    \caption{Evaluation of 2D common corruptions for the DNNs trained on ImageNet-100 with and without OpticsAugment. }
    \label{fig:common2d_modes}
\end{figure}


%%%%%%%%%%%%%%%%% DenseNet161 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_clean_\network.pdf}
    \caption{Highlighted: DenseNet clean (no augmentation)}
    \label{fig:common2d_modes_clean}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_opticsaugment_\network.pdf}
    \caption{Highlighted: DenseNet clean + OpticsAugment}
    \label{fig:common2d_modes_opticsaugment}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[trim=2cm 8.3cm 0.5cm 0cm,clip,width=0.9\linewidth]{figures/imagenet100-c/eval_rgb/labels_only_severity_split.pdf}
    \caption{2D common corruptions evaluated in Fig.~\ref{fig:common2d_modes_clean} and Fig.~\ref{fig:common2d_modes_opticsaugment}.}
\end{subfigure}
    \caption{Evaluation of 2D common corruptions for the DNNs trained on ImageNet-100 with and without OpticsAugment. }
    \label{fig:common2d_modes}
\end{figure}

%%%%%%%%%%%%%%%%% EfficientNet b0 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_clean_efficientnet.pdf}
    \caption{Highlighted: EfficientNet clean (no augmentation)}
    \label{fig:common2d_modes_clean}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_opticsaugment_efficientnet.pdf}
    \caption{Highlighted: EfficentNet clean + OpticsAugment}
    \label{fig:common2d_modes_opticsaugment}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[trim=2cm 8.3cm 0.5cm 0cm,clip,width=0.9\linewidth]{figures/imagenet100-c/eval_rgb/labels_only_severity_split.pdf}
    \caption{2D common corruptions evaluated in Fig.~\ref{fig:common2d_modes_clean} and Fig.~\ref{fig:common2d_modes_opticsaugment}.}
\end{subfigure}
    \caption{Evaluation of 2D common corruptions for the DNNs trained on ImageNet-100 with and without OpticsAugment. }
    \label{fig:common2d_modes}
\end{figure}

%%%%%%%%%%%%%%%%% ResNeXt50 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_clean_resnext50.pdf}
    \caption{Highlighted: ResNext50 clean (no augmentation)}
    \label{fig:common2d_modes_clean}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_opticsaugment_resnext50.pdf}
    \caption{Highlighted: ResNext50 clean + OpticsAugment}
    \label{fig:common2d_modes_opticsaugment}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[trim=2cm 8.3cm 0.5cm 0cm,clip,width=0.9\linewidth]{figures/imagenet100-c/eval_rgb/labels_only_severity_split.pdf}
    \caption{2D common corruptions evaluated in Fig.~\ref{fig:common2d_modes_clean} and Fig.~\ref{fig:common2d_modes_opticsaugment}.}
\end{subfigure}
    \caption{Evaluation of 2D common corruptions for the DNNs trained on ImageNet-100 with and without OpticsAugment. }
    \label{fig:common2d_modes}
\end{figure}


%%%%%%%%%%%%%%%%% MobileNet %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[h]
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_clean_mobilenet.pdf}
    \caption{Highlighted: MobileNet clean (no augmentation)}
    \label{fig:common2d_modes_clean}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/imagenet100-c/eval_rgb/report_acc_over_severitysplit_corruptions_opticsaugment_mobilenet.pdf}
    \caption{Highlighted: MobileNet clean + OpticsAugment}
    \label{fig:common2d_modes_opticsaugment}
\end{subfigure}
 \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[trim=2cm 8.3cm 0.5cm 0cm,clip,width=0.9\linewidth]{figures/imagenet100-c/eval_rgb/labels_only_severity_split.pdf}
    \caption{2D common corruptions evaluated in Fig.~\ref{fig:common2d_modes_clean} and Fig.~\ref{fig:common2d_modes_opticsaugment}.}
\end{subfigure}
    \caption{Evaluation of 2D common corruptions for the DNNs trained on ImageNet-100 with and without OpticsAugment. }
    \label{fig:common2d_modes}
\end{figure}
\fi


\iffalse
\begin{table}[h]
    \caption{Selection of pretrained models from pytorch vision and (RobustBench model zoos) with corresponding number of trainable parameters. The selected neural networks from RobustBench use a ResNet50.}
    \label{}    
    \centering
    \begin{tabular}{l l l}
    Architecture & Variants &  Parameter $[\times 10^6]$\\
    (AlexNet) &  & \\
    ConvNeXt & (tiny,small,base,large) & \\
    DenseNet & (161,169,201) & \\
    EfficientNet & (b0-b7) &\\
    Inception\_v3 & & \\
    MobileNet & (2,3) & \\ 
    MnasNet &  (0.5,0.75,1.0,1.3) & \\
    ShuffleNet &  &\\
    SqueezeNet & (1\_0,1\_1) &\\
    RegNetX & (400mf,800mf,1\_gf,3\_2gf,8\_gf) &\\
    RegNetY & (400mf,800mf,1\_gf,3\_2gf,8\_gf) &\\
    ResNet     &  (50,101,152) & \\
    ResNet (wide) &  (50,101) & \\
    ResNeXt     &  (50,101) & \\
    VGG &  (11,13,16,19) & \\
    \end{tabular}
    \centering
\end{table}
\fi

\iffalse 
% model list 
['alexnet', 'resnet18', 'resnet34', 'resnet50', 'resnet101', 'resnet152', 'resnext50_32x4d', 'resnext101_32x8d', 'wide_resnet50_2', 'wide_resnet101_2', 'vgg11', 'vgg11_bn', 'vgg13', 'vgg13_bn', 'vgg16', 'vgg16_bn', 'vgg19_bn', 'vgg19', 'squeezenet1_0', 'squeezenet1_1', 'inception_v3', 'densenet121', 'densenet169', 'densenet201', 'densenet161', 'mobilenet_v2', 'mobilenet_v3_large', 'mobilenet_v3_small', 'mnasnet0_5', 'mnasnet0_75', 'mnasnet1_0', 'mnasnet1_3', 'shufflenet_v2_x0_5', 'shufflenet_v2_x1_0', 'shufflenet_v2_x1_5', 'shufflenet_v2_x2_0', 'efficientnet_b0', 'efficientnet_b1', 'efficientnet_b2', 'efficientnet_b3', 'efficientnet_b4', 'efficientnet_b5', 'efficientnet_b6', 'efficientnet_b7',  'regnet_x_400mf', 'regnet_x_800mf', 'regnet_x_1_6gf', 'regnet_x_3_2gf', 'regnet_x_8gf', 'regnet_x_16gf', 'regnet_x_32gf', 
'regnet_y_800mf', 'regnet_y_1_6gf', 'regnet_y_3_2gf', 'regnet_y_8gf', 'regnet_y_16gf', 'regnet_y_32gf', 'vit_b_16','vit_b_32','vit_l_16','vit_l_32',\
'convnext_tiny','convnext_small','convnext_base','convnext_large']
\fi

\iffalse
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/eval_rgb/report_acc_over_severitysplit_corruptions.pdf}
    \caption{Accuracy for the different severities. Colors refer to the different corruptions from left to the right. The red diamonds show the accuracy for ConvNeXt\_base.}
    \label{fig:acc_vs_severity}
\end{figure}
\fi


